Friends with Costs and Benefits: Community Formation with Myopic, Boundedly-Rational Actors

In this paper we address how complex social communities emerge from local decisions by individuals with limited attention and knowledge. This problem is critical; if we understand community formation mechanisms, it may be possible to intervene to improve social welfare. We propose an interpretable, novel model for attributed community formation driven by resource-bounded individuals' strategic, selfish behavior. In our stylized model, attributed individuals act strategically in two dimensions: attribute and network structure. Agents are endowed with limited attention, and communication costs limit the number of active connections. In each time step, each agent proposes a new friendship. Agents then accept proposals, decline proposals, or remove friends, consistent with their strategy to maximize payoff. We identify criteria (number of stable triads) for convergence to some community structure and prove that our community formation model converges to a stable network. Ablations justify the ecological validity of our model and show that each aspect of the model is essential. Our empirical results on a physical world microfinance community demonstrate excellent model fits compared to baseline models.

==> sections/discussion.tex <==
We found that $\kappa=10$ was the best fit across all of our village dataset networks.
For the edge-sets we considered in the village microfinance data, this suggests that the considered interactions are not so socially costly that they are restricted to one's closest circle yet are too costly to be substantially broader.
That the best $\kappa$ is the same for hypothetical question edge sets as well as the factual question edge set suggests that survey respondents consider these interactions with equal social weight.
As our $\alpha$ and $\beta$ values represent population level preferences for attribute and structure respectively, a good fit on the observed networks may imply that our parameters reflect the preferences of the people in these networks.
If $\tau_v$ may take on a vector of values or any categorical value with more than two options, agents with high preferences for embeddedness and heterophily may form more robust networks as well.
